Monitoring the adoption of SPI-related best practices. An experience report

Software Process Improvement requires significant effort related not only to the identification of relevant issues and providing an adequate response to them, but also to the implementation and adoption of the changes. Best practices provide recommendations to software teams on how to address the identified objectives in practice, based on aggregated experience and knowledge. In the paper, we present the GEANT experience and observations from the process of adopting thebest practices, and present the setting we have been using.

==> results.tex <==
\section{How to identify key areas for improvements?}
\label{sec:results}

%OLD

%One of the key goals for analysis is to perform comparative ranking and clustering of topics based on their rating by participants of the survey. In the future, we plan to focus primarily on the areas where the greatest gains could be accrued in terms of practices improvements. The data collected so far significantly contributed to the selection of topics that should be promoted, worked on and supported through the improvement incentives.

%One of the goals for analysis was to identify the areas that deserve most attention and effort. The data collected so helped in the selection of topics that should be promoted, worked on and supported through the improvement incentives. Below, we provide comments on them:
 
%\begin{itemize}
%    \item The first candidate areas and specific goals are those for with the greatest diversity in the responses to related questions in the conducted survey in terms of satisfaction and expressed knowledge of associated practices. These are the topics where the benefit could be achieved with the least effort and by relying on the available internal expertise and through the harmonisation of knowledge and practices across teams. Although needs may vary from team to team, this harmonisation would contribute to mobility between teams due to the reconciliation of internal standards and, indirectly, external expectations. 

%    \item First, we focused on the areas in which the declared knowledge and satisfaction of the software teams was the most diversified. For those items, we can rely on the immediately available internal expertise of some teams, which reduces the effort needed for process improvement. Such harmonisation of processes among teams could additionally strengthen their collaboration.

%    \item Another issue refers to areas 
    %where the reaction is needed are those 
%    for which the survey scores were generally low or mediocre. These can be interpreted two-fold: either (1) the survey has identified a relevant topic that has been underestimated and has not been covered adequately, or (2) the topic is considered irrelevant by developers. To determine the actual status of these topics, teams and their leaders should be consulted. For that reason, it is useful at this point to establish a regular mechanism for collecting feedback from software teams. 
    %If a topic is to be incorporated, it may be necessary to change the current context, reformulate or change the strategic goals or enhance communication of existing ones. 
%    The apparent difficulty associated with these topics is the insufficient internal experience, so it may be necessary to look for external expertise and support to achieve the expected improvements.%, as well as to attain a wide mobilisation, as all teams need to improve in these areas.

 %   \item The third group of interest includes the areas with uniformly high marks. Here, we can expect relatively small improvements, even if the collected data is not completely accurate. High grades given by all teams may indicate that the reached level cannot or should not be further improved.%, and hint the lack the willingness and incentive to improve things further, as everyone thinks that everything in that area is good. Of course, senior-level management can propose or request improvements even in the areas where grades are consistently high.

%    \item In the third group are the areas where the marks are uniformly high. Here, the smallest gains can be expected, even if the obtained image is not completely accurate. Uniform high grades are an indication of the shared view that the reached level cannot or should not be raised further, and hint the lack the willingness and incentive to improve things further, as everyone thinks that everything in that area is good. Of course, senior-level management can propose or request improvements even in the areas where grades are consistently high.

\end{itemize}

%MW - I don't quite follow this part - it contains valuable recommendation, like for example the one to consult with management etc. But I think such recommendations are rather a part of the internal documents than a public paper?

%BM - this is generic of the proposed process and logic, with indications of convenient inflection points where  the higher management could intervene or be consulted. So I returned this to the paper. But wording could be changed or some additional explanations could be given if you feel uneasy with this...

%At this point, it is convenient to consult with the management that directs project activities within which software development is performed. Specifically, they can correct and further streamline the expert views articulated through the GSMM topics and the questionnaire used in the survey, as well as interpretations of responses. The convenience of this moment is additionally reflected in the availability of the thematic structure established by the GSMM team, data about teams' opinions about offered topics, as well as first-level filtering of topics, as described above. This gives the managers a set of choices and arguments that can help them make informed and optimal decisions. From the point of the enhancement of software engineering across G\'{E}ANT teams, this also contributes to strengthening the mandate to implement improvements and further engage software development teams.


%The instruments established to collect feedback from software teams should not be used just to address the dilemmas related to the selection of improvement areas. They could be also applied to get a response about the ongoing improvement initiatives and track the metrics that are relevant for the implementation of the GSMM. However, conducting extensive interview-based surveys, like the one described in Section~\ref{sec:process}, requires significant effort; at next stages, they could be supported with simpler and frequently run online questionnaires that focus on the key elements. %and include fewer questions and closed answer lists.
%These questions should be used to determine the needs and interests for potential new topics, track changes in indicators associated with already approved topics and even suggest and assess new indicators.

%Optionally, this approach could be taken even further by associating the indicators with maturity levels. Maturity is assessed against key capability and practice characteristics linked with the selected target areas at each level of the model. Maturity levels are typically established using a five-point Likert scale where the higher the level, the higher is the level of maturity. These progressive levels guide the planning and development of roadmaps. 
%It is good to use the same scale and general descriptions of levels as in other maturity models since this facilitates mixing or aligning of several related but distinct maturity models. With this, it is possible to determine the maturity level against a set of predefined criteria and to develop corresponding self-evaluation or certification tools. 
%As the subject of evaluation may demonstrate different maturity levels within individual areas and for different indicators, typically the lowest one found is used to determine the overall maturity. 
%Currently, there is no need for G\'{E}ANT to develop such a far-reaching maturity model. A future move in this direction would require reaching beyond G\'{E}ANT into an even larger base of software teams to capture the indicators and link their values to maturity levels.
%as this is the only way to justify the effort and produce stable and non-disputable indicators and levels. 
%Given the number of potential indicators and certain subjectivity in associating them with maturity levels, it is necessary to draw from the opinions and attitudes of a larger community to get non-disputable criteria. 
%The capture from a much larger group of actors and sources would also ensure better coverage of the diverse and heterogeneous software governance ecosystem. 
%Although other related standardisation processes and schemes and maturity models could additionally support this development, it is crucial to establish and employ a simple, inclusive and quality process in which the indicators and levels are produced and challenged. Again, a series of simple and low-effort online surveys could be used to iteratively establish and maintain the set of used indicators and maturity criteria.

%Observations/Results:
%\begin{itemize}
%    \item There is diversity in meeting the goals in G\'{E}ANT across teams and in various areas
%    \item a maturity model should capture the key areas, addressing the context, constraints and opportunities
%    \item objectives are not enough; they should be accompanied by directing guidelines; we call them ``best practices''
%    \item Best practices provide ``soft'' guidance on how to meet the specified goals; they should be derived from the goals they address
%    \item Best practices need to be structured (outline their resemblance to design patterns!)
%    \item Best practices should instruct 'what', rather than 'how'. How may be too specific. That activates the teams and ensures they adapt the BPs to their environment
%    \item Their level of details should be above procedures should be more general than procedures, but also address the context and constraints of the organisations
%\end{itemize}
